Interactivity x Explainability: Toward Understanding How Interactivity Can Improve Computer Vision Explanations

Explanations for computer vision models are important tools for interpreting how the underlying models work. However, they are often presented in static formats, which pose challenges for users, including information overload, a gap between semantic and pixel-level information, and limited opportunities for exploration. We investigate interactivity as a mechanism for tackling these issues in three common explanation types: heatmap-based, concept-based, and prototype-based explanations. We conducted a study (N=24), using a bird identification task, involving participants with diverse technical and domain expertise. We found that while interactivity enhances user control, facilitates rapid convergence to relevant information, and allows users to expand their understanding of the model and explanation, it also introduces new challenges. To address these, we provide design recommendations for interactive computer vision explanations, including carefully selected default views, independent input controls, and constrained output spaces.

==> 2_related_work_long.tex <==
\section{Related Work}
% Motivate explanations
Given the increasing ubiquity of AI \cite{singhal2023medpalm, ma2024medsam, huang2023plip, janai2020autonomous, michielssen2024baseball}, there exists a growing need for end-users to understand a model's behavior so they can appropriately trust and use the model.
To address this need, many XAI methods have been developed over the past decade across various subfields of AI (e.g., CV and robotics)~\cite{Lundberg2017shap, danilevsky2020nlpxai, lime, milani2024xrlsurvey, qian2021nlpxaiinterface} and across different domains (e.g., healthcare and climate science)~\cite{DeGrave2023auditing, antoniadi2021clinical, Lotsch2022Biomedicine, Singh2020Imaging, Smith2021ClinicalAI, Atakishiyev2021autonomous, Meteier2019AutomatedDriving, Machlev2022Energy, Mamalakis2022Climate}.
Historically, much work has focused on \textit{developing methods} to explain a model's outputs (e.g., answering \textit{``why did the model predict X?''}).
Recently, research has emerged at the intersection of XAI and Human-Computer Interaction (HCI) on \textit{evaluating how useful} explanation methods are for users with varying machine learning (ML) expertise \cite{nauta2023xaievalsurvey, jinli2022medxaihci, nazar2021medxaihci}. 
% (see \todo{ \cref{sec:problems}})

% However, these have predominately studied static explanations, whereas our work focuses on interactive explanations for computer vision.
%In this section, we first discuss works related to the types of computer vision explanations we study and current problems with static explanations (\cref{sec:cv_types,sec:problems}).
% Then, we highlight relevant research on interactivity in XAI and the types of interactive mechanisms we consider (\cref{sec:xai_interactive,sec:int_mech}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% What types of explanations do we use, include Figure 1
%\subsection{Types of Computer Vision Explanations}

\subsection{Types of Explanations}
% \label{sec:cv_types}
In this work, we focus on \emph{attribution-based} explanations, which compute a measure of importance by identifying the parts of an input that are critical for a model's decision \cite{goyal2019counterfacvis, miller2021contrastive} and have been the most developed method in XAI research thus far.
%Specifically, attribution-based explanations compute a measure of importance %(e.g., a 0-1 scale where a higher score indicates higher importance)
% for each item in the input (e.g., words, pixels).
% We study this class of explanations primarily because they have been most developed in XAI research thus far.
% Second, they attribute predictions at the level of pixels or image regions rather than at the level of similar images (as in the case of example-based explanations~\cite{koh2017influence,yeh2018representer}). This allows us to ask more uniform survey questions and perform fairer comparisons.
We discuss the following three types of attribution-based explanations: 
% heatmap-, concept-, and prototype-based explanations.

\subsubsection{Heatmap-based explanations} 
    typically generate a temperature heatmap over an input image that indicates the importance of each pixel or image region for the model's prediction~\cite{gradcam, lime, petsiuk2018rise, fong2017meaningful, brendel2019bagnet, simonyan2013deep, shitole2021sag, zeiler2014visualizing, Zhou2016CAM}. % (\cref{fig:cv_types}A).

\subsubsection{Concept-based explanations.} 
    Txplain a model's output using semantic concepts by assigning a numerical importance scores to each concept (e.g., +2.7 for ``wings'')~\cite{koh2020concept, ramaswamy2022elude, shukla2023cavli, zhou2018ibd}.% These explanations list a set of concepts that contribute to the model's prediction (e.g., ``wings'', ``bill'') and assign a numerical importance score to each concept (e.g., +2.7 for ``wings'').

\subsubsection{Prototype-based explanations} 
    learn a set of important image regions (i.e., prototypes) from training images \cite{chen2019protopnet, rymarczyk2022proto, kenny2023towards, nauta2021prototree, donnelly2022deformable, Nguyen2022team}.
    Given a new image, they then match its regions to the most similar prototypes from the learned set and report those regions alongside similarity scores as contributing to the model's prediction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Problems with the static CV explanations
\subsection{Problems with Static CV Explanations}
%\label{sec:problems}
CV explanations are typically static explanations.
However, several user studies in XAI and in Information Visualization have highlighted 3 main issues with static CV explanations:
% We group these issues into three overarching problems: 1. information overload, 2. gaps between semantics and pixel-level information, and 3. limited means for user-driven exploration.

\subsubsection{Information Overload.}
    Prior work has found that the amount of information in CV explanations can be overwhelming to users. With heatmaps, users often want to view only the ``extremes'' of a heatmap and thus find intermediate colors distracting~\cite{kriglstein2014gameplay, xia2018heatmap, blignaut2010heatmap}. For concepts, users reported feeling overwhelmed by the number of items displayed \cite{kim2023hmhta, ramaswamy2023overlooked}, which often is the number of annotated objects in a dataset (e.g., $1197$ in the Broden dataset~\cite{bau2017netdissect}). Similarly, prototypes can require many regions to explain a model well enough \cite{kim2016criticisms}.

\subsubsection{Semantic-Pixel Gap.}
    Prior work suggests users often find it difficult to connect image regions to the represented object and vice versa. For concepts, users have difficulty identifying the objects or attributes in the images \cite{ramaswamy2023overlooked}. With heatmaps and prototypes, users struggle to discern what objects correspond to the highlighted regions \cite{kim2023hmhta, blignaut2010heatmap}.\looseness-1

\subsubsection{Limited means for user-driven exploration.}
    Finally, it has been found that users desire insight into why an explanation was produced. Although attribution-based explanations show \textit{what} image regions are important, they do not explain \textit{why} they are important \cite{miller2021contrastive, wachter2018contrastive}. However, Kim et al. \cite{kim2023hmhta} found that users wanted to know why certain regions were considered important when using heatmap-, concept-, and prototype-based explanations. This is in part because users often do not understand how an explanation is computed \cite{bekri2020expapproach}. However, another reason is that users often lack the ability to \emph{probe} these explanations beyond the static presentation.


% Interactivity in explainable AI, this is where the reviewers said we needed better coverage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interactivity in XAI applications}
\label{sec:xai_interactive}
The explanations discussed in \todo{\Cref{sec:cv_types}} have primarily been developed as static explanations; thus, there were limited opportunities for users to interact with the displayed information.
While the problems discussed in \todo{\Cref{sec:problems}} could be at least partially mitigated by adjusting the amount of information in the static explanation on a case-by-case basis, interactivity has been identified as an effective \cite{sundar2012interactiveeffective, kim2017infovisinteractivity, sundar2010interactivitycustom, srinivasan2019interactive} and customizable \cite{sundar2010interactivitycustom, srinivasan2019interactive} way for people to interact with and understand data, particularly for large datasets \cite{boggust2022embedding, yi2007interaction}.

% Interactive mechanisms we focus on and why we chose them
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Types of Interactive Mechanisms}
\label{sec:int_mech}

==> todos.tex <==
% NOTE: 
    % If you add any text to the paper, use \new{} 
        % This is so that we can keep track of changes in case the review process asks for that
        % For the clean camera ready we just set the color to back, and if they want us to track changes we use the blue
        % It's not necassary to use this for very minor changes

% 1) Limitations
    % There is a rich literature on interactivity x info viz that we haven't engaged with deeply so it's unclear to what extent our findings and recommendations are specific to explanations. If we don't have room or space to do this, I suggest that we acknowledge it as a path for future work to bring in more of these learnings and study if they are applicable in XAI domains, particularly for CV explanations

% 2) Figures 
    % Bar chart needs to be replaced with "Real" ones; I edited it in Photoshop so it would take less space 

% 3) Quant results 
    % We need to include the statistical results for the quantitative section (including effect size, etc), in addition to p-values 

%  4) Formatting 
    % Reference formatting and missing names 
    % Inconsistencies in capitalization of presentation type names and explanation type names
        % For example concept-based or concepts in section 2 but Concept-based in section 3
        % We also say "concept version", "concepts", or "concept-based" interchangeably, but not sure if it's important to keep those consistent as well
        % same with "Static" vs "static"
    % Inconsistencies in quotation mark usage
        % sometimes `` '' and other times " " 
        % We should also be consistent about whether \textit{} is inside or outside of quotations; same with punctuations
    % Appendix
        % Given that we have appendix A & B at the end of the paper, I think the supplemental materials should start from C 
        % We should also revisit what we include in the supplemental materials

% 5) Finally there are comments throughout the Overleaf document that would be good to address 

% Todos from before: 
    % There are some remaining todos here from before: https://docs.google.com/document/d/1rQFRGrygD9tC6NVoABn1DRwWCJcq2CCT2w-lJ33D-8Q/edit?tab=t.0#heading=h.eztswuv04jet
    % We should be strategic about what we add and make sure we don't add too much/increase the length of the paper.
